Stratifying systems over hereditary algebras

This paper deals with stratifying systems over hereditary algebras. In the case of tame hereditary algebras we obtain a bound for the size of the stratifying systems composed only by regular modules and we conclude that stratifying systems can not be complete. For wild hereditary algebras with more than 2 vertices we show that there exists a complete stratifying system whose elements are regular modules. In the other case, we conclude that there are no stratifing system over them with regular modules. In one example we built all the stratifying systems, with a specific form, having maximal number of regular summads.

==> biblio.tex <==
@article{Ba,
   author    = "Baer, D."
    year      = "(1989)".
    title     = "A note on wild quiver algebras and tilting modules".
    journal   = "Comm. in Algebra".
    volume   = "17:"
    %number   = "",
    pages    = "751-757".
}

@article{ES,
  author =       "Erdman, K., Sáenz, C. "
   year =        "(2003)."
  title =        "On standardly stratified algebras."
  journal =      "Comm. in Algebra."
  volume =       "31:",
  %number =       "10",
  pages =        "3429-3446."
  %year =         "1905",
}

 
@article{einstein,
  author =       "Albert Einstein",
  title =        "{Zur Elektrodynamik bewegter K{\"o}rper}. ({German})
                 [{On} the electrodynamics of moving bodies]",
  journal =      "Annalen der Physik",
  volume =       "322",
  number =       "10",
  pages =        "891--921",
  year =         "1905",
}

